Open Source Software Field Research: Spanning Social and Practice Networks for Re-Entering the Field

Sociotechnical research increasingly includes the social sub-networks that emerge from large-scale sociotechnical infrastructure, including the infrastructure for building open source software. This paper addresses these numerous sub-networks as advantageous for researchers. It provides a methodological synthesis focusing on how researchers can best span adjacent social sub-networks during engaged field research. Specifically, we describe practices and artifacts that aid movement from one social subsystem within a more extensive technical infrastructure to another. To surface the importance of spanning sub-networks, we incorporate a discussion of social capital and the role of technical infrastructure in its development for sociotechnical researchers. We then characterize a five-step process for spanning social sub-networks during engaged field research: commitment, context mapping, jargon competence, returning value, and bridging. We then present our experience studying corporate open source software projects and the role of that experience in accelerating our work in open source scientific software research as described through the lens of bridging social capital. Based on our analysis, we offer recommendations for engaging in fieldwork in adjacent social sub-networks that share a technical context and discussion of how the relationship between social and technically acquired social capital is a missing but critical methodological dimension for research on large-scale sociotechnical research.

==> paper/0_authors.tex <==

%no clue on order so feel free to change
\author{Sean Goggins}
\orcid{0000-0002-4331-147X}
\affiliation{%
  \institution{University of Missouri}
  \streetaddress{}
  \city{}
  \state{MO}
  \postcode{}
  \country{USA}
}
\email{outdoors@acm.org}

\author{Kevin Lumbard}
\orcid{0000-0001-9306-3040}
\affiliation{%
  \institution{University of Nebraska at Omaha}
  \streetaddress{6001 Dodge Street}
  \city{Omaha}
  \state{NE}
  \postcode{68182}
  \country{USA}
}
\email{klumbard@unomaha.edu}


\author{Caifan Du}
\orcid{https://orcid.org/0000-0003-2538-607X}
\affiliation{%
  \institution{University of Texas at Austin}
  \streetaddress{1616 Guadalupe Street}
  \city{Austin}
  \state{TX}
  \postcode{78701-1213}
  \country{USA}
}
\email{cfdu@utexas.edu}

\author{Karthik Ram}
\orcid{0000-0002-0233-1757}
\affiliation{%
  \institution{University of California, Berkeley}
  \streetaddress{}
  \city{Berkeley}
  \state{CA}
  \postcode{94720}
  \country{USA}
}
\email{karthik.ram@berkeley.edu}

\author{James Howison}
\orcid{0000-0002-5702-149X}
\affiliation{%
  \institution{University of Texas at Austin}
  \streetaddress{1616 Guadalupe Street}
  \city{Austin}
  \state{TX}
  \postcode{78701-1213}
  \country{USA}
}
\email{jhowison@ischool.utexas.edu}

\author{Matt Germonprez}
\orcid{0000-0003-2326-5901}
\affiliation{%
  \institution{University of Nebraska at Omaha}
  \streetaddress{6001 Dodge Street}
  \city{Omaha}
  \state{NE}
  \postcode{68182}
  \country{USA}
}
\email{germonprez@gmail.com}

% The default list of authors is too long for headers.
\renewcommand{\shortauthors}{M. Germonprez et al.}
